Revisiting Convergence of AdaGrad with Relaxed Assumptions

In this study, we revisit the convergence of AdaGrad with momentum (covering AdaGrad as a special case) on non-convex smooth optimization problems. We consider a general noise model where the noise magnitude is controlled by the function value gap together with the gradient magnitude. This model encompasses a broad range of noises including bounded noise, sub-Gaussian noise, affine variance noise and the expected smoothness, and it has been shown to be more realistic in many practical applications. Our analysis yields a probabilistic convergence rate which, under the general noise, could reach at (\tilde{\mathcal{O}}(1/\sqrt{T})). This rate does not rely on prior knowledge of problem-parameters and could accelerate to (\tilde{\mathcal{O}}(1/T)) where (T) denotes the total number iterations, when the noise parameters related to the function value gap and noise level are sufficiently small. The convergence rate thus matches the lower rate for stochastic first-order methods over non-convex smooth landscape up to logarithm terms [Arjevani et al., 2023]. We further derive a convergence bound for AdaGrad with mometum, considering the generalized smoothness where the local smoothness is controlled by a first-order function of the gradient norm.

==> Related_work.tex <==
\section{Related works}

SGD and its adaptive variants has been a target of intense interest in the last decade; we invite the readers for \citep{bottou2018optimization,ruder2016overview} for an overview, and we limit our discussions to the most relevant literature in the sequel.

\paragraph{Adaptive methods for non-convex optimization} Numerous of works mainly studied the convergence guarantees of adaptive methods in an expectation view. \citet{li2019convergence} provided a rate of $\tilde{\mathcal{O}}(1/\sqrt{T})$ for AdaGrad-Norm with a delayed step-size that is independent from current stochastic gradient but required knowledge of smoothness parameter. Meanwhile, \citet{ward2020adagrad} obtained a rate of $\tilde{\mathcal{O}}(1/\sqrt{T})$ for AdaGrad-Norm without prior knowledge of problem parameters but assuming a uniform bound of gradients. \citet{faw2022power} studied AdaGrad-Norm in the case of affine variance noise and achieved a desired convergence rate of $\tilde{\mathcal{O}}(1/\sqrt{T})$ without assuming uniformly bounded gradients. More recently, \citet{alina2023on} established a convergence bound for AdaGrad-Norm and its acceleration version on quasar-convex smooth problems. The element-wise version of AdaGrad was studied by \citet{zou2019sufficient} with a heavy-ball or Nesterov style momentum. \citet{zaheer2018adaptive} and \citet{chen2018convergence} also proved convergence bounds for Adam-type algorithm. Later, \citet{defossez2020simple} improved the convergence rate for Adam and AdaGrad with a better dependency on the momentum parameter, specifically of order $\mathcal{O}((1-\beta)^{-1})$. Another recent work by \citet{guo2021novel} made progress in allowing for improved convergence rates with increasing momentum parameter, but again required knowledge of the smoothness parameter. In parallel, \citet{rakhlinconvergence} studied Adam convergence behavior on non-convex generalized smooth problems under the bounded noise variance assumption. More recently, \citet{zhou2023win} introduced the Nesterov-alike-acceleration into Adam and AdamW and justified the convergence superiority over non-accelerated version. 

\paragraph{High probability convergence bounds} \citet{ghadimi2013stochastic} provided a high probability convergence result for vanilla SGD with the knowledge of smoothness and sub-Gaussian noise. Later, \citet{harvey2019tight} established a high probability bound for Projected SGD with bounded noise on strongly-convex non-smooth Lipschitz functions. There exist some works for establishing high probability bounds for adaptive methods. \citet{zhou2018convergence} and \citet{ward2020adagrad} provided high probability bounds for AMSGrad and AdaGrad with sub-Gaussian noise and bounded noise, respectively, although neither of these bounds were optimal to the probability margin. \citet{li2020high} considered AdaGrad with a delayed step-size and obtained a high probability bound with the knowledge of smoothness. More recently, \citet{kavis2022high} made progress in obtaining an convergence bound that is optimal to the probability margin for AdaGrad-Norm, assuming uniformly bounded gradients and sub-Gaussian noise. Additionally, \citet{attia2023sgd} relaxed the uniformly bounded condition and obtained a bound adaptive to the noise level for AdaGrad-Norm under affine variance noise. In parallel, \citet{alina2023high} also established an optimal high probability bound for both scalar and element-wise versions of AdaGrad with sub-Gaussian noise. Recently, some other high probability convergence results emerged for Cilpped SGD on both convex and smooth non-convex cases under heavy-tail assumptions \citep{cutkosky2021high,sadiev2023high,nguyen2023high}.


